The multi-thermal and multi-stranded nature of coronal rain

In this work, we analyse coordinated observations spanning chromospheric, TR and coronal temperatures at very high resolution which reveal essential characteristics of thermally unstable plasmas. Coronal rain is found to be a highly multi-thermal phenomenon with a high degree of co-spatiality in the multi-wavelength emission. EUV darkening and quasi-periodic intensity variations are found to be strongly correlated to coronal rain showers. Progressive cooling of coronal rain is observed, leading to a height dependence of the emission. A fast-slow two-step catastrophic cooling progression is found, which may reflect the transition to optically thick plasma states. The intermittent and clumpy appearance of coronal rain at coronal heights becomes more continuous and persistent at chromospheric heights just before impact, mainly due to a funnel effect from the observed expansion of the magnetic field. Strong density inhomogeneities on spatial scales of 0.2"-0.5" are found, in which TR to chromospheric temperature transition occurs at the lowest detectable scales. The shape of the distribution of coronal rain widths is found to be independent of temperature with peaks close to the resolution limit of each telescope, ranging from 0.2" to 0.8". However we find a sharp increase of clump numbers at the coolest wavelengths and especially at higher resolution, suggesting that the bulk of the rain distribution remains undetected. Rain clumps appear organised in strands in both chromospheric and TR temperatures, suggesting an important role of thermal instability in the shaping of fundamental loop substructure. We further find structure reminiscent of the MHD thermal mode. Rain core densities are estimated to vary between 2x10^{10} cm^{-3} and 2.5x10^{11} cm^{-3} leading to significant downward mass fluxes per loop of 1-5x10^{9} g s^{-1}, suggesting a major role in the chromosphere-corona mass cycle.

==> table1.tex <==
\ProvidesFile{table1.tex}%
 [2003/12/12 5.2/AAS markup document class]%
 
\begin{deluxetable}{ccccc}
\tabletypesize{}
\tablecaption{Average values for both datasets}
\tablewidth{0pt}
\tablehead{
\colhead{Instrument} & \colhead{Dataset} & \colhead{Width} & \colhead{Length} & \colhead{Blobs} \\
\& filter & & \colhead{[arcsec]} & \colhead{[arcsec]} & \colhead{/ min}
}
\startdata
CRISP - H$\alpha$ & 1 & 0.30 $\pm$ 0.09 & 3.85 $\pm$ 5.77 &  5.0  \\
SOT - \ion{Ca}{2}~H & 2 & 0.61 $\pm$ 0.17 & 1.05 $\pm$ 0.51 & 9.7 \\
SJI - 2796 & 2 & 0.80 $\pm$ 0.20 & 2.49 $\pm$ 1.97 & 2.6 \\
SJI - 1330 & 2 & 0.70 $\pm 0.15$ & 1.75 $\pm$ 1.35 & 3.7 \\ 
SJI - 1400 & 2 & 0.81 $\pm 0.17$ & 1.76 $\pm$ 1.26 & 4.6 \\ 
AIA - 304 & 2 & 1.56 $\pm 0.15$ & 10.8 $\pm$ 6.5 & 2.2 \\
AIA - 304 & 1 & 1.40 $\pm 0.70$ & 12.7 $\pm$ 9.2 & 1.2 \\
AIA - 171 & 1 & 2.45 $\pm 0.81$ & 5.5 $\pm$ 5.2  & 1.2 \\
AIA - 193 & 1 & 2.69 $\pm 1.07$ & 7.4 $\pm$ 4.6 & 1.2 
\enddata
\tablecomments{Averages are calculated over all detected blobs in both datasets. Row order is set according to increasing temperature. For dataset 1 the measurements are limited only to the rain detected in loops 1 and 2. For dataset 2 the measurements are limited to the loop shown in Fig.~\ref{fig8}. While each measurement is itself an average value over a large quantity (see section~\ref{methods}) and therefore has its own standard deviation, the standard deviation shown here for widths (lengths) is simply taken over the set of blob widths (lengths). The last column provides the number of blobs detected per minute for each dataset, which implies dependence over the FOV over which this detection is carried. For the \textit{SST}, the detection is done over a small part of its FOV (roughly 5\arcsec$\times$17\arcsec), which is much smaller than the FOV for the \textit{SDO} data of the same dataset (see Fig.~\ref{fig3}). For \textit{Hinode} the projected area over which the the rain is detected is roughly twice that of \textit{SST}.
\label{table1}}
\end{deluxetable}

\endinput
